A Survey of Fusion Frames in Hilbert Spaces

Fusion frames are a very active area of research today because of their myriad of applications in pure mathematics, applied mathematics, engineering, medicine, signal and image processing and much more. They provide a great flexibility for designing sets of vectors for applications and are therefore prominent in all these areas, including e.g. mitigating the effects of noise in a signal or giving robustness to erasures. In this chapter, we present the fundamentals of fusion frame theory with an emphasis on their delicate relation to frame theory. The goal here is to provide researchers and students with an easy entry into this topic. Proofs for fusion frames will be self-contained and differences between frames and fusion frames are analyzed. In particular, we focus on the subtleties of fusion frame duality. We also provide a reproducible research implementation.

==> figures/old/fusiogram_discussion.tex <==
\begin{rem}
{\bf \xxl Internal Discussion:}
\begin{itemize}
\item 
{\xxl Noch was: $A = 0$? Für dier Fusin Frames und/ oder dem global Frame?
fuer den globalen, also das, dessen positive f in der mitte der figure abgebildet sind. \\
- Die einzelnen lokalen frames sind keine frames für den ganzen Raum, also haben alle $A=0$. 
Aber der globale Frame sollte ein Frame für den ganzen Raum sein, sonst machen wir etwas falsch. 
Und der Fusion Frame sollte auch ganz gute Frame Bounds haben. \\
{\xxl {\bf New:} Apropos: Für das globale frame bzw. den fusion frame sollte die Interpolation vollkommen egal sein. } \\
{Warum nur in 'der Mitte der Figure'?}

\item {\clara frage: ich tu hier wirklich nur "rausschneiden", also ein segment in der Figure ist so wie hier dargestellt nicht die Addition von 6 frames-1 segment. 
{\xxl ?? Was meinst Du ?? Jedes lokale Frame sollte 'unabhängig' sein, und die Werte sollen in die volle Matrix eingetragen werden, im Überlapppungsbereich können dann Werte von mehreren lockal Frames stehen. }
Wenn ich das aber mache, gibt es auch vernünftige frame bounds. {\xxl Wenn Du was machst? Wenn Du $\Psi_i$ statt $\Phi_i$ nimmst? }
{\clara wart, ich schreib dir mal den ablauf auf, weil das mach ich ja. } {\xxl Okay}

\begin{enumerate}
\item DGT/FWT von input sig
\item expanden auf [L x L] {\xxl Wie?} {\clara upsampling nach $a$, bestimmen des f-Vektors, und dann innerhalb der f-Baender mit derselben f wiederholen}
\item dann: das ist der punkt wo ich mir nicht sicher war, entweder alle 6 frames aufaddieren, oder eben nicht. {\xxl Warte, schon aufaddieren, aber vor (2). (Eigentlich den Mittelwert nehmen, im seltenen Fall, wo der selbe Punkt von mehrern Frames beschreiben wird.)  Wenn Du zuerst interpolierst, bekommen die 'echten' Werte weniger Relevanz.} mach ich 
{\xxl Dann geht das aber mit dem Upsamplen nicht mehr 'gut', weil dann da mitunter zwischen den DGT werten ein FWT-Wert steht, deswegen meinte ich plumpes Spline-Interpolieren. } {\clara das mach ich danach. aber ich komm ja nie auf meine Dimensionen wenn ich das nicht mach, also plakativ: ich komm nicht von 64 auf 128, sonst; ich koennte die werte aber einfach wiederholen, so wie ich es auch fuer die frequenzen mache. dann gibt es aber halt auch nix zum interpolieren.}
{\xxl Nein, nicht wiederholen. Also für die DGT $M_{ak,bl} = DGT(k,l)$ ...  }
\item passt, aber wie komm ich dann zur begruendung, welche sequenzen raus geschnitten werden? {\xxl Das ist unsere Wahl .... }
\item passt, dann mach ich mit allen aufaddiert, aber schon interpoliert, nochmal? {\xxl Unklar .... }
das loest halt das, was du oben geschrieben hast, mit den wavelet werten zwischen den DGT werten nicht...aber ich kenne alle positionen, ich koennte die werte, die nicht in der Naehe einer Ueberlappung sind, anders gewichten, quasi ausfaden
{\xxl einfach mit dem Standard SPline interpolation machen?  \verb+fillmissing+  } mir geht es um den schritt davor. ich muss ja zuerst einmal die t-f ebene irgendwie aufspannen. also halt, die koeffizienten, die ich hab sinnvoll verteilen.
{\xxl Ja, aber Du brauchst nicht mehr.}
{\clara wenn ich eine wavelet-[7 x 64] (cell, also unterschiedliche laengen) array hab, und dann nichts tue, zwischen was interpolier ich dann? das ist ja in der form gar nicht sparse}
{\xxl Ich hätte vermutet, dass das ein Füllung in 2D ist, ... sonst haben wir ein Problem ja. }
{\clara ich versteh glaub ich nicht, was du meinst;}
{\xxl Ich hoffe, dass das _fillmissing_ auch interpoliert, wenn nicht in jeder ZTeite bzw. Spalte was steht. } {\verb_fillmissing_ kann das nicht a-priori .... ich schau' noch. Okay, man muss zuerst eine Richtung dann die andere machen: A = [1 NaN 1 NaN; 0 1 NaN NaN; NaN NaN NaN NaN;1 NaN 1 0]
B = fillmissing(A,'spline',1)
C = fillmissing(B,'spline',2)}
{\clara ja, das hab ich eh, ich glaub wir schreiben aneinander vorbei}
{\xxl Wenn Du interpolierst brauchst Du kein Upsampling, etc..  }
{\clara also, ich bleib bei der DGT. von der krieg ich eine matrix [8 x 24] oder so aehnlich. die sollte aber [L x L] (wenn ich jetzt nicht zwischen pos. und neg. f unterscheide) sein. es ist klar, dass ich nicht L x L Werte habe (also Annahme: L >> 24), die fehlenden Werte interpolier ich. Aber wenn ich das ohne irgendwas mache, hab ich keinerlei t-f Korrespondenz mehr in was auch immer da dann raus kommt. }
{\clara ah, ja, das haut hin}
{\clara aber dazu muss ich trotzdem vorher meine stuetzstellen ja richtig verteilt haben, }
{\xxl Richtig!}
{\clara naja und damit ich das machen kann, muss ich mMn in irgendeiner Form upsamplen}
{\xxl Jein, das Problem: Upsampling interpoliert bereits. }
{\clara naja, dabei halt schon nan einfuegen}
{\xxl Ja, aber das ist kein Upsamling, oder? Also statt Zeile (1 1 1) -> (1 NaN Nan 1 Nan Nan 1 Nan Nan) }
{\clara fuer mich schon -.-', ist das irgendwie definiert?
das hab ich nicht gewusst
}
{\xxl Siehe \url{https://en.wikipedia.org/wiki/Upsampling}. Du hast recht, wenn Du statt Nullen NaNs nimmst, ist das Upsamplen (einfach eine Inverse zu Downsampling). Die Interpolation muss - wie ich eigentlich dachte - nicht unbedinbgt dabei sein. }
{\xxl Aha, also Du brauchst keine FFT o.ä. }
{\xxl Okay, dann machst Du keine Interpolation, sondern nur ein Upsampling in der oben beschriebene Wiese, das passt. (Allerdings müssen wir dann noch immer aufpassen, wie man die Stütztstellen der anderen einträgt. Denn NaN + 5 = NaN. }
{\xxl Ich muss weg ... Kinder! Morgen 9:00 }
{\clara sheesh, ja passt}
{\xxl 9:30? ;-) } {\clara besser}
{\xxl Und ich glaueb wir haben an enander vrobei geredet bzw. ich bin von etwas falsche ausgegangen. Lösch' bitte die Sqachen, die jetzt kalr sind, und lass' nur die noch offenen Fragen (auch von mir drinnen). }
{\clara passt, bis morgen}
{\clara ach, nicht so schlimm, das kann ich lösen. also einfach neue indizes zuweisen, dazwischen mit nan auffuellen, wuerd passen?}
{\clara warte. wenn ich eine Folge [s1 nan s2 nan ,..., sn] hab, und die dann auf eine zweite, [nan t1 nan t2 nan ,..., tn, nan], dann will ich ja in unserem Fall eh [s1 t1 s2 t2 , ... sn, tn] haben, oder? vielleicht reden wir nur}
\end{enumerate}
{\xxl Ich schreib gleich die Fragen / Kommentare durnter ;-) 
(2) sollte ein Expnanden der Koeffizienten, nicht der Frame Sequenzen sein. Und sollte insbesondere etwas keine volle STFT machen....
}
\end{itemize}
\end{rem}


{\xxl   {\bf Wait: } The analysis coefficients of both} frame sequences were then extended to the full $[L \times L]$ time-frequency grid. {\xxl Wir wollen aj nicht die frame sequences erweitern, sondern die Koeffizienten interpolieren????  } 

{\clara Dazu muss ich sie aber zuerst erweitern, aus der fwt krieg ich irgendwas mit dimension [7 x 64] raus, und aus der DGT, je nachdem, sowas wie [24 x 8]}
{\xxl Ja, passt. Das sollte dann in die $L \times L$-Matrix eingetragen werden. }


%OLD STUFF+++++++++++++++++++++++++++++++++++++++++++++++

%{\clara  
%Assigning a time and frequency index to each frame element $\psi^{(i)}_k$ in $Q_i$, according to $\psi^{(i)}_k = (t^{i}_k, f^{i}_k)$, is straight forward, due to the uniform sampling grid. The local frames can then be defined as a sequence of local frames $\Phi^{(i)} = \psi^{(i)}_k$, such that $(t^{i}_k, f^{i}_k) \in Q_i$. \\
%For Figure~\ref{frame_sequences}, we, somewhat arbitrarily, opted to plot those $Q_i$ that correspond to overlapping regions in Figure~\ref{fig_fusiogram2}. Figures~\ref{ol_t} and ~\ref{ol_f} represent the overlapping regions in time and frequency respectively.
%and are optically dominated by the dyadic wavelet structure, with the Gabor frame enhancing the local energy, indicated as yellow dots, at those points where its diagonal elements intersect with the time-frequency sampling grid. In Figure~\ref{ol_tf}, to the left, where the regions that overlap in both, time and frequency are shown, the contribution of the Gabor structure (and the absence of this contribution, in the Figure to the right), is evident.\\

%\begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[trim={10cm 0cm 10cm 0}, width=\textwidth]
%         {fusio2_ol_normalized.png}
%         \caption{ Coefficients of the local frames of a fusion frame. }
%         \label{fig_fusio2}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[trim={10cm 0 10cm 0}, width=\textwidth]{fusio2_ol_normalized_norm.png}
%         \caption{Norm of the fusion frame coefficients with the same subspaces.}
%         \label{fig_fusio2_norm}
%     \end{subfigure}
%     \caption{Depicted to the left is a plot of the local frame coefficients {\xxl interpolated to a full time-frequency plane $L \times L$ (see text). The } fusion frame comprised of six subspaces, covered by wavelet and a Gabor frames, {\xxl  alternatively - starting with a wavelet frame in the top left corner. }
%     Coefficients in the overlapping region were {\clara summed {\xxl \bf averaged? } }
     %The subspaces are constructed from local frames retrieved from the fast wavelet transform using a Daubechies wavelet of order $8$ and iteration depth $J=6$ and a discrete Gabor transfom using a Gaussian window ($a, b = 1$). 
%     They have been arranged on a rectangular grid, in a fashion that resembles conventional time-frequency representations, allowing for some overlap, as described in the text. The overlapping subspaces are indicated as white lines.  
%     Depicted to the right are the norms of the analysis vectors $p_i$.
%     They are arranged in the same way, therefore resulting in overlapping regions for positive and negative frequencies. {\xxl \bf Bitte hier auch die Mittelung durchf\"uhren, also durch die Gewichte dividieren.  }}\label{fig_fusiogram2}
%\end{figure}

%\begin{figure}
%\centering
%\begin{subfigure}[b]{0.45\textwidth}
%\includegraphics[trim={8.5cm 4.0cm 8cm 3.3cm},clip,scale =.1]{ol_t_normalized.png}
%\subcaption{Elements that overlap in time}\label{ol_t}
%\end{subfigure}
%\hfill
%\begin{subfigure}[b]{0.45\textwidth}
%\includegraphics[trim={8.5cm 4.0cm 8cm 3.3cm},clip,scale =.1]{ol_f_normalized}
%\subcaption{Elements that overlap in frequency}\label{ol_f}
%\end{subfigure}
%\vspace{3cm}%
%%
%\centering
%\begin{subfigure}[b]{0.7\textwidth}
%\includegraphics[trim={8.5cm 4.0cm 8cm 3.3cm},clip,scale =.1]{ol_tf_normalized.png}
%\subcaption{{\clara Elements that overlap in time and frequency}}\label{ol_tf}
%\end{subfigure}
%\end{figure}\label{frame_sequences}
%
%}}

\section{For Discussion: Fusiogram} 

While this certainly will be the topic of future research and a much more systematic approach, we display an example plot, comprising local frames derived from the fast wavelet transform (FWT)~\cite{mallat}, using a Daubechies wavelet~\cite{daubechies} and iteration order {\clara $J=10$}, in Figure~\ref{fig_fusogramdirect}. In Figure~\ref{fig_fusogramnorm}, we plot the norms of the analysis vectors $p_i  = \pi_{W_i} f$ as in Figure~\ref{fig_coefsnorm_ana}.

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[trim={10cm 0cm 10cm 0}, width=\textwidth]
         {fig5_fusiogram_wl.png}
         \caption{ Coefficients of the local frames of a fusion frame. }
         \label{fig_fusogramdirect}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[trim={10cm 0 10cm 0}, width=\textwidth]{fig5_norm_matrix_ana.png}
         \caption{Norm of the fusion frame coefficients with the same subspaces.}
         \label{fig_fusogramnorm}
     \end{subfigure}
     \caption{Depicted to the left is a plot of the local frame coefficients of a fusion frame comprising six subspaces. Those coefficents that were considered in the overlapping region were summed. 
     The subspaces are constructed from local frames retrieved from the fast wavelet transform using a Daubechies wavelet of order $8$ and iteration depth $J=10$. They have been arranged on a rectangular grid, in a fashion that resembles conventional time-frequency representations, allowing for some overlap, as described in the text. The overlapping subspaces are indicated as white lines.  
     Depicted to the right are the norms of the analysis vectors $p_i$.
     They are arranged in the same way as before, therefore resulting in overlapping regions for positive and negative frequencies.}\label{fig_fusogram}
\end{figure}

{\clara We arrive at this representation in three steps. Firstly, the layout of the resulting global fusion frame, that is, the number of local frames to be used and their arrangement in a matrix-like structure, along with their overlap in the two dimensions, must be passed as input arguments. Currently, only layouts featuring uniform row- and column numbers are supported (this might change). In a second step, the input signal is preprocessed to match that layout in both, time and frequency. Thirdly and finally, the local frames' associated operators are applied to the signal segments, with their summation (according to the layout and specified overlap) yielding the final global fusion frame.}\\
 
{\clara The fusion frame at hand comprises six local FWT frames of the same dimension $L_i=1024$ and $K_i = J + 1$ frequency channels per local frame. Its layout was chosen to feature two rows comprising three FWT tiles each. We have defined an overlap, specified as $ol = 0.1$ throughout, for display purposes (solely). The dimensions of the fusiogram arrangement  are given as $L=n_c L_i- (n_c -1 ) o_{lc} L_i$, with $n_c$ the specified number of horizontally arranged fusion frames, the "columns", and $o_{lc}$ their overlap factor.
We would also like to consider a frequency overlap, analogously, $K=n_r K_i- (n_r -1 ) o_{lr} K_i$, with $n_r$ the number of desired "rows", $o_{lf}$ their overlap factor, and $K$ the total number of frequency channels.} 
\\

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[trim={6cm 1cm 8cm 2cm},clip,width=\textwidth]
         {input_upper_ol.png}
         \caption{Input signal upper tiles}
         \label{fig_coefsdirect}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[trim={6cm 1cm 8cm 2cm},clip,width=\textwidth]{input_lower_ol.png}
         \caption{Input signal lower tiles } 
         \label{fig_coefsnormmat}
     \end{subfigure}
             \caption{The (random) input signals, with values ranging from $]0, 1[$, used as an input to the upper and lower subspace tiles of the fusiogram, respectively, after being low- and highpass filtered. 
         The respective start and end points per segment after temporal splitting (i.e. the overlapping regions) are indicated via black lines. }\label{inputsignal}
\end{figure}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[trim={6cm 1cm 8cm 2cm},clip,width=\textwidth]
         {fig7_fb_freqresp_font.png}
         \caption{Frequency response of the filter bank.}
         \label{fig_fb}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[trim={6cm 1cm 8cm 2cm},clip,width=\textwidth]{fig7_dgt_coefs_font.png}
         \caption{Discrete Gabor coefficients of the input signal.} 
         \label{fig_coefsdgt}
     \end{subfigure}
             \caption{Depicted to the left is the frequency response of the filterbank used. To the right are the discrete Gabor coefficients of the middle, that is, highest energy, signal segments according to Figure~\ref{inputsignal}.}\label{inputsignal_freq}
\end{figure}


{\clara 
We consider a  random signal $f$ (with values ranging from $]0, 1[$) windowed by a Gaussian window as an input. 
To be able to process the input signal in the desired constellation, some preprocessing needs to be applied. Specifically, the input signal was split into overlapping segments in time, according to $o_{lc}$ and $L_i$, as depicted in Figure~\ref{inputsignal}. To align the local frames across frequency, we did a similar approach on the frequency side. For all three signals, we calculated a low-pass and a high-pass signal with overlap $o_{lr}$ as described above, and shifted the high-pass signal downwards (towards frequency $0$), and the low-pass signal upwards in frequency. The frequency response of the filter bank used is depicted in Figure~\ref{fig_fb}, with the resulting discrete Gabor coefficients of the middle segments of the input signal depicted in Figure~\ref{fig_coefsdgt}. Then, we transferred both signals to time domain again, \sout{down sampled by $\frac{M_i}{M} \le 2$}, and applied the two local wavelet systems.}\\ 

%{\xxl \bf Here $M_i$ is only the frequency direction, and not both, being in contradiction to Table 1. Change one}
%{\xxl F\"ur die Anzahl der Elemente im Global Frame muss man ja den Overlap nicht abziehen. Für die Frequenz-Auflösung macht das aber Sinn (sollte aber dann einen anderen Namen haben?). Siehe Idee unten. 
%
% Warum macht es für die Anzahl der lokalen Frame-Element keinen Sinn: Der globale Frame hat $M = \sum M_i$ Elemente, also die einfache Summe. Wenn wir nicht nur die Koeffizienten der überlappendedn Bereich betrachten, sondern dort die Summe der Elemente annehmen, dann haben wir ein Problem bzgl. Rekonstruktion, weil das dann eben keine lokalen Frames mehr sind.  
%}

{\clara Each of the local frames was then calculated as the analysis coefficients of $f$. The fusion frame was then constructed from the local frames, via summation at the time  frequency indices corresponding to the layout specified above. While to ensure reconstruction, it is necessary to store the original fusion frame coefficients, for display purposes, prior to summing up, coefficients lower than $-200$ were set to zero. This can be seen as first attempt to combine fusion frames containing frame elements smaller than $L$, as for example hinted at in \cite{caku13}.  \\}


%{\clara From this fusiogram representation, it is equally possible to select overlapping regions $Q_i$ in the time frequency plane, depicted in Figure~\ref{overlapping_regions} exemplarily for those regions of the representation in Figure~\ref{fig_fusogram} that overlap either in time, frequency, or both. Assigning a time and frequency index to each frame element $\psi^{(i)}_k$ in $Q_i$, according to $\psi^{(i)}_k = (t^{i}_k, f^{i}_k)$, possibly taking into account those of the input signal, is straight forward. From there, the local frames can then be defined as a sequence of local frames $\Phi^{(i)} = \psi^{(i)}_k$, such that $(t^{i}_k, f^{i}_k) \in Q_i$. \\
%}


%\begin{figure}
%\centering
%\begin{subfigure}[b]{0.45\textwidth}
%\includegraphics[trim={8.5cm 4.0cm 8cm 3.3cm},clip,scale %=.1]{ol_time.png}
%\subcaption{Elements that overlap in time}
%\end{subfigure}
%\hfill
%\begin{subfigure}[b]{0.45\textwidth}
%\includegraphics[trim={8.5cm 4.0cm 8cm 3.3cm},clip,scale %=.1]{ol_freq}
%\subcaption{Elements that overlap in frequency}
%\end{subfigure}
%\vspace{3cm}%


%\centering
%\begin{subfigure}[b]{0.7\textwidth}
%\includegraphics[trim={8.5cm 4.0cm 8cm 3.3cm},clip,scale %=.1]{ol_time_freq.png}
%\subcaption{Elements that overlap in time and frequency}
%\end{subfigure}
%%\subfigure[text]{
%%\includegraphics[width=.225\textwidth]{file}
%%}

%\caption{Elements of Figure~\ref{fig_fusogram} that overlap in %time, in frequency, or both. }\label{overlapping_regions}
%\label{fig:whatever}
%\end{figure}


%{\xxl Note that the wavelet transforms corresponds not to the full length $L$, but to $L_i$, which also reduces their freuqnecy range ...  {\bf Schau' mal, ob das stimmt, bitte. Ist das so? Haben wir nicht so wie bei der Gabor tarnsformation einfach nur weniger Punkte auf frequenz-Seite?}}{\clara nein, weil das wavelet system explizit fuer die Laenge $L_i$ aufgestellt ist und einfach so wie es ist drauf addiert wird. ich kontrolliere die laenge ja indirekt ueber die iterationstiefe der mallat-filterbank-baum struktur $J$, aber ich versteh, dass das evtl. missverstaendlich formuliert ist. ansonsten, ja, je kleiner $J$, desto kleiner die Anzahl an Frequenzkanaelen.}
%{\xxl Das ist klar, aber sind es weniger über den selben Frequenzbereich verteilt, oder kommen die weniger weit hinauf. Wenn ich mich jetzt nicht ganz irre, bedeutet weniger Skalen auch einen kleineren frequnz-Bereich, oder?
%Also9 ist der Frequnzbereich von $L_i$ kleiner als der von $L$?}
%{\clara nein, der algorithmus lauft so, dass er den gesamten f-bereich, den das eingangssignal halt hat (gegeben durch seine laenge, dann), einmal hoch- und tiefpass filtert, weitere iterationen fuehren dann nur dazu, dass die "frequenzaufloesung", also halt die kanalanzahl groesser wird, quasi das signal wird besser approximiert, aber nicht der abstand zwischen $f_min$ und $f_max$. mir (aber sonst niemandem in der mathe gruppe) hilft das block diagramm immer sehr: \url{http://ltfat.org/doc/wavelets/fwt.html}. das ist eh eigentlich der grund, warum ich das eingangssignal bearbeite. }
%{\xxl Danke! Das ist jetzt klar.}

%{\xxl Die Wavelet transform deckt immer den ganzen Frequenzbereich ab, daher macht Modulation keinen Sinn. Wir müßten auch auf wenige Punkte kommen. 

%{\bf Idee} ??.... Fourier transformation -> Filterung (in diesem Fall auf zwei Bereiche) -> zwei Signale (im Frequenz-Bereich): $y_1$ (Tiefbass), $y_2$ (Hochpass) -> $z_1$ = $y_1$, $z_2$ = $y_2$ geshiftet nach unten. Rekonstruktion auf zeitbereich, downsampling um 2.
%{\xxl
%Also zum Beispiel (wenn wir die $M$-Formel wieder belegen möchten ....
%{\color{blue}
%" To align the local frames across frequency, we did a similat approach om the frequency side. For all three signal we calculated a low-pass and a high-pass signal with overlap as described above , we modulated the high-pass signal down (towards frequency $0$), transferred both signal to time domain again, downsampled by $\frac{M_i}{M} \le 2$, and then applied the two local wavelet systems."}

%Das wäre quasi der erste Schritt in Mallat doppelt nur einmal umgedreht ?

%  Der Overlap in der Zeit wäre aber somit größer .... aber da kommen wir nicht herum (unschärfe) ... ausser wir wollen dann die Koeffizienten ausschneiden. 
  
%  }
%\\

%{\xxl \bf Frage: Summieren wir nur die Koeffizienten (und da wahrscheinlich nur die Absolutbeträge) oder summieren wir tatsächlich die Frame Elemente? Ich bin für ersteres, sonst verlieren wir den Fusion Frame Bezug (weil ja die Summe von zwei Frame Elementen aus zwei lokalen Frames dann in keinem lokalen Frame mehr sind. Also so umformulieren, warte ich mache es :}
%{\clara wirklich nur die elemente, also skalare einzeleintraege}
%{\xxl DIe Summe der Skalar-produkte? 
%Wir betrachten zwar $\psi^{(i)_j}$ und $\psi^{(i+1)_j}$ als unterschiedliche lokale Frame-elemente, stellen aber $\left< f, \psi^{(i)_j}\right> + \left< f, \psi^{(i+1)_j}\right> = \left< f, \psi^{(i)_j} \psi^{(i+1)_j}\right> $ dar, bzw. deren Absolutbeträge ja?
%}
%{\clara nein, frame elemente desselben lokalen frames werden nie miteinander summiert. } {\xxl Ja, aber von zwei verschiedenen. Das Resultat ist in keinem der beiden lokalen frames mehr, in general. Was ich meine: Wir müssen die original Koeffizienten uns merken, sonst geht die Rekonstruktion schief.}


%{\clara wegen absolutbetrag: momentan summiere ich nicht die absolutbetraege. weil ich letztlich vektoraddition beim konzipieren im kopf gehabt hab. die ist aber derweil eh kein sinnvolles konzept und es ist natuerlich kein problem, das zu aendern...}
%{\xxl Aber wir plotten die Absolutbeträged, ja?} {\clara ja}
%{\xxl Okay, danke. Jetzt klar.} Lassen wir das noch da stehen



\subsection{Future Questions}

{\xxl F\"ur sp\"ater: K\"onnten wir f\"ur allgemeine Subspaces Ihr Zentrum in der Zeit-Frequenz-Ebene bestimmen? Und k\"onnten wir $\pi_{W_i} \psi_{k}^(j)$ etwa zum Beispiel summieren und dann in der TF-Ebene darstellen?}
{\clara haengt davon ab, was du mit "allgemeine subspaces" meinst. einfach beliebige kombinationen? rein geometrisch kann ich den mittelpunkt von sowas jetzt schon bestimmen, etwa als schnittpunkt der diagonalen ueber das rechteck in der t-f ebene, die sie aufspannen, den kann man dann natuerlich gewichten o.ae. aber so meinst du es wahrscheinlich nicht?
zum zweiten, sicherheitshalber: die orthogonale projektion auf $W_i$ der lokalen frame vektoren, also einfach die analyse koeffizienten?
}
{\xxl Wie gesagt: F\"ur sp\"ater.

Und ich wei\ss nicht .... $\pi_{W_i} f$, wobei $f$ wei\ss es Rauschen ist, und das ein paar Mal?

* Plot higher diemnsions fusion frames: Use \verb:TMAP: or \verb:t_SNE: or similar?

}



\end{document}


==> figures/old/fusiogram_text.tex <==

While this will be the topic of future research and a much more systematic approach, we display an example plot, comprising local frames derived from the fast wavelet transform (FWT)~\cite{mallat}, using a Daubechies wavelet~\cite{daubechies} and iteration order $J=6$, in Figure~\ref{fig_fusogramdirect}. In Figure~\ref{fig_fusogramnorm}, we plot the norms of the analysis vectors $p_i  = \pi_{W_i} f$.
 
 To arrive at this representation, we instantiated a fusion frame comprising six local FWT frames of the same dimension $L_i=128$. The layout of the representation was chosen to feature two rows comprising three FWT tiles each. The overlap was specified as $ol = 0.1$ throughout for display purposes, thus, 
yielding a global frame representation for dimension $L=n_c L_i- (n_c -1 ) o_l L_i$, with $n_c$ the specified number of horizontally arranged fusion frames, the "columns", and $o_l$ their overlap factor.
{\clara , and analogously, $M=n_r M_i- (n_r -1 ) o_l M_i$, with $n_r$ the number of desired "rows" and $M$ the total number of global  elements.}
{\xxl \bf F\"ur die Anzahl der Elemente im Global Frame muss man ja den Overlap nicht abziehen. Also den Satz einfach streichen?}

For each of these local frames, their analysis matrix 
%was calculated and (pointwise)
is applied to the input signal, depicted in Figure~\ref{inputsignal}.
%{\xxl and the absolute value on a lograithmical scale \bf ??? Yes, is this what we did ??}
%{\clara nein, ganz stupide einfach drauf multipliziert}

  
% {\xxl \bf Die Analyse in Figure~\ref{inputsignal} schaut komisch aus. Auch wenn wir DWT's zusammensetzen würde ich mir in der Mitte viel Energie erwarten, am Rand wenig. Die 'Spuren' in den Bildern sind auch komisch, ich w\"urde mir ind er Mitte einm typische Nullstellen-Verteilung erwatene, siehe etwa \url{https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9030834} Fig.2 oben - dort wo kien Signal ist. }
The random input signal (with values ranging from $]0, 1[$) was windowed by a Gaussian window,
%, corresponds to a periodization of the function $g(x) = \exp^{-\pi \frac{x.^2}{tfr}}$, with a time-frequency ratio $\text{tfr} = 100$, 
chosen such that the window covers the whole signal range of interest and for display purposes, see Fig. \ref{inputsignal}. 

%\begin{figure}
         %\includegraphics[trim={10cm 0cm 10cm 0}, %width=\textwidth]
         %{fig6_input_subplot}
         %\caption{The real parts of the (random) input signals, with values ranging from $]0, 1[$, used as an input to the upper and lower subspace tiles of the fusiogram, respectively, after exponential modulation. {\xxl \bf Ich sehe keine Modulation.}
         %{\clara ich bild hier aber auch nur den realteil ab und moduliere komplex mit $\exp^{j\dots}$}
         %{\xxl Trotzdem müßte man einen Frequenzschift sehen.}
         %%The two signals have the same amplitude range. {\clara man koennte auch die andere figure im topfolder nehmen, fig6inputsignal.png, da sind beide signale im selben koordinatensystem dargestellt, ich bin nicht sicher, was besser ist} {\xxl Ja.} 
         %Temporal splitting points are indicated via black lines %{\xxl \bf ... aber warte, hier sollte es ja eine Überlappung geben, oder} and the whole-point even Gaussian window applied is indicated via black dashed lines. {\clara nein, hier noch nicht, die ueberlappung entsteht ja erst beim aufaddieren der analysekoeffizienten des signals}
  %       {\xxl ?? Aber mit der Formel ober $L = ...$ geht sich das ja nur aus, wenn wir hier auch dieselb Überlappung haben. Sonst haben wir ja hier $L/3$ Dimension und oben mehr .... }
 %        {\clara ich verstehs nicht. in der formel oben ist der overlap schon eingerechnet, also $L_{frame} < L_{signal}$ wegen dem overlap. und wegen der modulation: ich hab eine gegenprobe gemacht, mit ref_dgt.m aus der LTFAT, da sieht man fuer weisses rauschen auch nichts.}
         
%         }\label{inputsignal}
%\end{figure}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[trim={6cm 1cm 8cm 2cm},clip,width=\textwidth]%{ana_final_transp_font.png}
         {input_upper.png}
         \caption{Input signal upper tiles}
         \label{fig_coefsdirect}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[trim={6cm 1cm 8cm 2cm},clip,width=\textwidth]{input_lower.png}
         %{fig4_subspace_index_norm.png}
         \caption{Input signal lower tiles } 
         \label{fig_coefsnorm}
     \end{subfigure}
             \caption{The real parts of the (random) input signals, with values ranging from $]0, 1[$, used as an input to the upper and lower subspace tiles of the fusiogram, respectively, after exponential modulation. {\xxl \bf Ich sehe keine Modulation.}
         {\clara ich bild hier aber auch nur den realteil ab und moduliere komplex mit $\exp^{j\dots}$}
         {\xxl Trotzdem müßte man einen Frequenzschift sehen.}
         %The two signals have the same amplitude range. {\clara man koennte auch die andere figure im topfolder nehmen, fig6inputsignal.png, da sind beide signale im selben koordinatensystem dargestellt, ich bin nicht sicher, was besser ist} {\xxl Ja.} 
         Temporal splitting points are indicated via black lines {\xxl \bf ... aber warte, hier sollte es ja eine Überlappung geben, oder} and the whole-point even Gaussian window applied is indicated via black dashed lines. {\clara nein, hier noch nicht, die ueberlappung entsteht ja erst beim aufaddieren der analysekoeffizienten des signals}
         {\xxl ?? Aber mit der Formel ober $L = ...$ geht sich das ja nur aus, wenn wir hier auch dieselb Überlappung haben. Sonst haben wir ja hier $L/3$ Dimension und oben mehr .... }
         {\clara ich verstehs nicht. in der formel oben ist der overlap schon eingerechnet, also $L_{frame} < L_{signal}$ wegen dem overlap. und wegen der modulation: ich hab eine gegenprobe gemacht, mit refdgt.m aus der LTFAT, da sieht man fuer weisses rauschen auch keinen f-shift.}}\label{inputsignal}
\end{figure}


%In LTFAT, the FWT (and all other time-frequency associated frames) are implemented such that they cover per default the whole frequency range from zero up to the input sampling frequency. 
To be able to order the subspaces according to their time-frequency position we adjusted the input signal
 rather than modifying the local frames.
To achieve temporal localization, we segmented the input signal $f$ in three portions of length $L$, corresponding to the envisioned layout of the representation (i.e. with time on the abscissa and frequency displayed on the ordinate). For fusion frames within the same column, the same signal segment was used. Here, the overlap described above, is used.

This can be seen as first attempt to be able to combine fusion frames containing frame elements smaller than $L$, as for example hinted at in \cite{caku13}.  \\
To align the local frames across frequency, the input signals were modulated %in Fourier transform-like fashion,
-  i.e. they were multiplied - by  $\exp^{2\pi i \frac{i_{min}}{L}}$, with $i_{min}$ derived from their relative coordinates within the global fusion frame representation, the difference between $M$ and $M_i$. 
%{\xxl \bf unclear ....  $K = 6$ hier? Könntest Du das noch genaue beschreiben, siehe auch untern}
For the successive wavelet transforms, the full wavelet system was used.\\

{\xxl Note that the wavelet transforms corresponds not to the full length $L$, but to $L_i$, which also reduces their freuqnecy range ...  {\bf Schau' mal, ob das stimmt, bitte. Ist das so? Haben wir nicht so wie bei der Gabor tarnsformation einfach nur weniger Punkte auf frequenz-Seite?}}{\clara nein, weil das wavelet system explizit fuer die Laenge $L_i$ aufgestellt ist und einfach so wie es ist drauf addiert wird. ich kontrolliere die laenge ja indirekt ueber die iterationstiefe der mallat-filterbank-baum struktur $J$, aber ich versteh, dass das evtl. missverstaendlich formuliert ist. ansonsten, ja, je kleiner $J$, desto kleiner die Anzahl an Frequenzkanaelen.}
{\xxl Das ist klar, aber sind es weniger über den selben Frequenzbereich verteilt, oder kommen die weniger weit hinauf. Wenn ich mich jetzt nicht ganz irre, bedeutet weniger Skalen auch einen kleineren frequnz-Bereich, oder?
Also9 ist der Frequnzbereich von $L_i$ kleiner als der von $L$?}
{\clara nein, der algorithmus lauft so, dass er den gesamten f-bereich, den das eingangssignal halt hat (gegeben durch seine laenge, dann), einmal hoch- und tiefpass filtert, weitere iterationen fuehren dann nur dazu, dass die "frequenzaufloesung", also halt die kanalanzahl groesser wird, quasi das signal wird besser approximiert, aber nicht der abstand zwischen $f_min$ und $f_max$. mir (aber sonst niemandem in der mathe gruppe) hilft das block diagramm immer sehr: \url{http://ltfat.org/doc/wavelets/fwt.html}. das ist eh eigentlich der grund, warum ich das eingangssignal bearbeite. }
\\

{\xxl \bf Frage: Summieren wir nur die Koeffizienten (und da wahrscheinlich nur die Absolutbeträge) oder summieren wir tatsächlich die Frame Elemente? Ich bin für ersteres, sonst verlieren wir den Fusion Frame Bezug (weil ja die Summe von zwei Frame Elementen aus zwei lokalen Frames dann in keinem lokalen Frame mehr sind. Also so umformulieren, warte ich mache es :}
{\clara wirklich nur die elemente, also skalare einzeleintraege}
{\xxl DIe Summe der Skalar-produkte? 
Wir betrachten zwar $\psi^{(i)_j}$ und $\psi^{(i+1)_j}$ als unterschiedliche lokale Frame-elemente, stellen aber $\left< f, \psi^{(i)_j}\right> + \left< f, \psi^{(i+1)_j}\right> = \left< f, \psi^{(i)_j} \psi^{(i+1)_j}\right> $ dar, bzw. deren Absolutbeträge ja?
}
{\clara nein, frame elemente desselben lokalen frames werden nie miteinander summiert.
warte, ich mach es implementationsnaeher, da tu ich mir leichter: ich hab eine Matrix \verb+A=zeros(L,M);+ und ich kenne die start und end indices fuer jede lokale frame matrix $a_i$, d.h. \verb+A(f_start:f_end, t_start:t_end) = + \\
\verb+A(f_start:f_end, t_start:t_end)\plus a_i;+ }

{\clara wegen absolutbetrag: momentan summiere ich nicht die absolutbetraege. weil ich letztlich vektoraddition beim konzipieren im kopf gehabt hab. die ist aber derweil eh kein sinnvolles konzept und es ist natuerlich kein problem, das zu aendern...}
{\xxl Aber wir plotten die Absolutbeträged, ja?} {\clara ja}

{\xxl Für später: Könnten wir für allgemeine Subspaces Ihr Zentrum in der Zeit-Frequenz-Ebene bestimmen? Und könnten wir $\pi_W_i \psi_{k}^(j)$ etwa zum Beispiel summieren und dann in der TF-Ebene darstellen?}
{\clara haengt davon ab, was du mit "allgemeine subspaces" meinst. einfach beliebige kombinationen? rein geometrisch kann ich den mittelpunkt von sowas jetzt schon bestimmen, etwa als schnittpunkt der diagonalen ueber das rechteck in der t-f ebene, die sie aufspannen, den kann man dann natuerlich gewichten o.ae. aber so meinst du es wahrscheinlich nicht?
zum zweiten, sicherheitshalber: die orthogonale projektion auf $W_i$ der lokalen frame vektoren, also einfach die analyse koeffizienten?
}
{\xxl Wie gesagt: F\"ur sp\"ater.

Und ich weiß nicht .... $\pi_{W_i} f$, wobei $f$ weißes Rauschen ist, und das ein paar Mal?
}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[trim={10cm 0cm 10cm 0}, width=\textwidth]
         %{fusionframe+signals.png}
         {fig5_tfplots1.png}
         %\caption{Overlapping frame coefficient matrices}
         \caption{ Coefficients of the local frames of a fusion frame and a random signal. }
         \label{fig_fusogramdirect}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[trim={10cm 0 10cm 0}, width=\textwidth]{fig5_tfplots_norm.png}
         %{fusionframe+signalsnorm.png}
         \caption{Norm of the fusion frame coefficients with the same subspaces.}
         \label{fig_fusogramnorm}
     \end{subfigure}
     \caption{Depicted to the left is a plot of the local frame coefficients of a fusion frame comprising six subspaces overlapping in the time-frequency plane. We analyze the random signal depicted in figure~\ref{inputsignal}. The subspaces are constructed from local frames retrieved from the fast wavelet transform using a Daubechies wavelet of order $8$ and iteration depth $J=6$. They have been arranged on a rectangular grid, in a fashion that resembles conventional time-frequency representations, allowing for some overlap, as described in the text. The overlapping subspaces are indicated as white lines. 
     %Depicted to the right are the sum of the norms %{\clara as obtained from analysis of each subspace coefficient matrix $[K_i \times L_i]$ by $K_i$ vectors $f_i = [1, 1, \dots, 1]$} of length $L_i$.  
     Depicted to the right are the norms of the analysis vectors $p_i$.
     They are arranged in the same way as before, therefore resulting in overlapping regions for positive and negative frequencies.}\label{fig_fusogram}
\end{figure}



DISCUSSION 21/11/22

%their analysis matrix 
%was calculated and (pointwise)
%is applied to the input signal. 
%{\xxl  For the regions, which are considered to be in the overlapping regions the analysis coefficients are added. The logarithmically scaled absolute values of the result is}  depicted in Figure~\ref{inputsignal}.
%{\xxl and the absolute value on a lograithmical scale \bf ??? Yes, is this what we did ??}
%{\clara nein, ganz stupide einfach drauf multipliziert}

  
% {\xxl \bf Die Analyse in Figure~\ref{inputsignal} schaut komisch aus. Auch wenn wir DWT's zusammensetzen würde ich mir in der Mitte viel Energie erwarten, am Rand wenig. Die 'Spuren' in den Bildern sind auch komisch, ich w\"urde mir ind er Mitte einm typische Nullstellen-Verteilung erwatene, siehe etwa \url{https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9030834} Fig.2 oben - dort wo kien Signal ist. }


%\begin{figure}
         %\includegraphics[trim={10cm 0cm 10cm 0}, %width=\textwidth]
         %{fig6_input_subplot}
         %\caption{The real parts of the (random) input signals, with values ranging from $]0, 1[$, used as an input to the upper and lower subspace tiles of the fusiogram, respectively, after exponential modulation. {\xxl \bf Ich sehe keine Modulation.}
         %{\clara ich bild hier aber auch nur den realteil ab und moduliere komplex mit $\exp^{j\dots}$}
         %{\xxl Trotzdem müßte man einen Frequenzschift sehen.}
         %%The two signals have the same amplitude range. {\clara man koennte auch die andere figure im topfolder nehmen, fig6inputsignal.png, da sind beide signale im selben koordinatensystem dargestellt, ich bin nicht sicher, was besser ist} {\xxl Ja.} 
         %Temporal splitting points are indicated via black lines %{\xxl \bf ... aber warte, hier sollte es ja eine Überlappung geben, oder} and the whole-point even Gaussian window applied is indicated via black dashed lines. {\clara nein, hier noch nicht, die ueberlappung entsteht ja erst beim aufaddieren der analysekoeffizienten des signals}
  %       {\xxl ?? Aber mit der Formel ober $L = ...$ geht sich das ja nur aus, wenn wir hier auch dieselb Überlappung haben. Sonst haben wir ja hier $L/3$ Dimension und oben mehr .... }
 %        {\clara ich verstehs nicht. in der formel oben ist der overlap schon eingerechnet, also $L_{frame} < L_{signal}$ wegen dem overlap. und wegen der modulation: ich hab eine gegenprobe gemacht, mit ref_dgt.m aus der LTFAT, da sieht man fuer weisses rauschen auch nichts.}
         
%         }\label{inputsignal}
%\end{figure}

%\begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[trim={6cm 1cm 8cm 2cm},clip,width=\textwidth]%{ana_final_transp_font.png}
%         {input_upper.png}
%         \caption{Input signal upper tiles}
%         \label{fig_coefsdirect}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[trim={6cm 1cm 8cm 2cm},clip,width=\textwidth]{input_lower.png}
%         %{fig4_subspace_index_norm.png}
%         \caption{Input signal lower tiles } 
%         \label{fig_coefsnorm}
%     \end{subfigure}
%             \caption{The real parts of the (random) input signals, with values ranging from $]0, 1[$, used as an input to the upper and lower subspace tiles of the fusiogram, respectively, after exponential modulation. {\xxl \bf Ich sehe keine Modulation.}
%         {\clara ich bild hier aber auch nur den realteil ab und moduliere komplex mit $\exp^{j\dots}$}
%         {\xxl Trotzdem müßte man einen Frequenzschift sehen.}
         %The two signals have the same amplitude range. {\clara man koennte auch die andere figure im topfolder nehmen, fig6inputsignal.png, da sind beide signale im selben koordinatensystem dargestellt, ich bin nicht sicher, was besser ist} {\xxl Ja.} 
%         Temporal splitting points are indicated via black lines {\xxl \bf ... aber warte, hier sollte es ja eine Überlappung geben, oder} and the whole-point even Gaussian window applied is indicated via black dashed lines. {\clara nein, hier noch nicht, die ueberlappung entsteht ja erst beim aufaddieren der analysekoeffizienten des signals}
%         {\xxl ?? Aber mit der Formel ober $L = ...$ geht sich das ja nur aus, wenn wir hier auch dieselb Überlappung haben. Sonst haben wir ja hier $L/3$ Dimension und oben mehr .... }
%         {\clara ich verstehs nicht. in der formel oben ist der overlap schon eingerechnet, also $L_{frame} < L_{signal}$ wegen dem overlap.
%         {\xxl \bf Genau, aber jedes lokale Frame hat die Dimension $L_i$ und nicht $\frac{L}{3} = \frac{L=3 L_i- (2) o_l L_i}{3} = L_i - \frac{2}{3} o_l L_i $. Das müssen wir daher mit einem Signal der Dimension $L_i$ beschicken, wa sheißt dass sich die Signal bereits überlappen müssen. }
%         }}\label{inputsignal}
%\end{figure}







%In LTFAT, the FWT (and all other time-frequency associated frames) are implemented such that they cover per default the whole frequency range from zero up to the input sampling frequency. 
%To be able to order the subspaces according to their time-frequency position we adjusted the input signal
% rather than modifying the local frames.
%To achieve temporal localization, we segmented the input signal $f$ in three portions of length $L$, corresponding to the envisioned layout of the representation (i.e. with time on the abscissa and frequency displayed on the ordinate). For fusion frames within the same column, the same signal segment was used. Here, the overlap described above, is used.
%{\color{blue}
%" To align the local frames across frequency, we did a similat approach om the frequency side. For all three signal we calculated a low-pass and a high-pass signal with overlap as described above , we modulated the high-pass signal down (towards frequency $0$), transferred both signal to time domain again, downsampled by $\frac{M_i}{M} \le 2$, and then applied the two local wavelet systems."}
%This can be seen as first attempt to combine fusion frames containing frame elements smaller than $L$, as for example hinted at in \cite{caku13}.  \\


%
%{\clara{\textbf{Clara: confirm that it is not $0, \dots J-1$ or similar}}}. Alignment with the frequency axis was achieved by replicating the thus obtained time-aligned coefficients within their respective frequency channels, according to the pre-determined downsampling factor ($b_{DGT} = \frac{L}{M}$ in the DGT case, and $b_{WL} = \frac{1}{2^{J_i}}$, with $J_i = 0,\dots, J$ in the wavelet case). \\
%{\xxl 
%This is solved algorithmically by first creating a $L \times L$- matrix $M$ consisting only of \verb:NaN: values, 'not-a-number'. 
%$$}
%
%{\clara To discuss: \\
%The resulting frames were then added
%}

%In Figure~\ref{fig_fusio2}, we represent a fusion frame as the superposition of overlapping local frames, specifically a wavelet and a Gabor transform, on a two dimensional time-frequency grid. The norms of its rows are displayed in Figure~\ref{fig_fusio2_norm}.%In those representations, lighter colors correspond to higher energy coefficients and the signal energy is spread amongst more coefficients for the Gabor than for the wavelet case. As a consequence, in Figure~\ref{fig_fusio2}, the structure of the wavelet frame appears visually more pronounced.\\

%We have chosen the time-frequency regions $Q_i$ to be {\bf ......} with a a symmetric overlap $o_l = 0.1L$. Those $Q_i$ that are plotted by white rectangles in Figure~\ref{fig_fusiogram2}. 

% Figures~\ref{ol_t} and ~\ref{ol_f} represent the overlapping regions in time and frequency respectively.
%As local frame we have chosen wavelet frames using a Daubechies wavelet of order $8$ andGabor frames ($a, b = 1$) using a Gaussian window. {\xxl Why high redundancy? Why not a standard Gabor?} The wavelet frame was generated from a fast wavelet transform. 
%{\clara To arrive at the full $[L \times L]$ representation of the dyadic sampling grid depicted here, upsampling in  time and frequency was applied. {\xxl \bf Unclear. How ? See above ? }
% The coefficients from the local frames are mapped to those points that corresponds (best) to the time-frequency positions of the local frame. This is doable for wavelet and Gabor frames. 
%
%For those frames the mapping from frame element to time-frequency is straight-forward. 
%{\xxl \bf We have to deal with the negative frequencies, I propose to use them conjugate symmetric.}

%A random signal (value range $]0,\dots 1[$), windowed by a Gaussian window {\xxl plus sinusoid ???}, was used as an input, see Figure \ref{fig:signal}. 
%In Figure \ref{fig_fusio2_norm} we plot the norm of the fusion frame coefficients as in the Figure before. 


%\begin{figure} 
%\includegraphics[trim={7cm 2cm 7cm 2cm}, clip, width=\textwidth]{fusiogram.png}
%\caption{Upper tile: the input signal used: a sequence of random numbers with values ranging from $]0, \dots 1[$, windowed by a Gaussian window, and a sinusoid with $f_c = \frac{f_s}{4}=128$. Middle tile: the fusiogram, generated from a wavelet and a Gabor frame sequence. Only positive frequencies are displayed. Lower tile: the global fusiogram. The frame bounds are below numerical precision, i.e. $A~0$. 
%{\clara \textbf{du wolltest noch mehrfach den untersten plot? soll ich das noch machen und dann die $f$ des sinus variieren?}}
%}
%\label{fig:fusiogram}
%\end{figure}
